Archives of Photographic PLates for Astronomical USE (APPLAUSE) Digitisation of astronomical plates and their integration into the International Virtual Observatory

The Archives of Photographic PLates for Astronomical USE (APPLAUSE) project is aimed at digitising astronomical photographic plates from three major German plate collections, making them accessible through integration into the International Virtual Observatory (IVO). Photographic plates and related materials (logbooks, envelopes, etc.) were scanned with commercial flatbed scanners. Astrometric and photometric calibrations were carried out with the developed PyPlate software, using Gaia EDR3 data as a reference. The APPLAUSE data publication complies with IVO standards. The latest data release contains images and metadata from 27 plate collections from the partner institutes in Hamburg, Bamberg, and Potsdam, along with digitised archives provided by Tautenburg, Tartu, and Vatican observatories. Altogether, over two billion calibrated measurements extracted from about 70,000 direct photographic plates can readily be used to create long-term light curves. For instance, we constructed the historic light curve of the enigmatic dipping star KIC 8462852. We found no evidence of previously assumed variations on timescales of decades in our light curve. Potential uses of APPLAUSE images for transient sources can be appreciated by following the development of the nova shell of GK Per (1901) over time and the change in brightness of two extragalactic supernovae. The database holds about 10,000 spectral plates. We made use of objective prism plates to follow the temporal changes of Nova DN Gem through 1912 and 1913, highlighting an outburst in early 1913.

==> applause_plot_alt.tex <==
\pagebreak

\onecolumn
\section{Mollweide maps of observations per archive} 


\begin{figure}[h]
\begin{tabular}{cc}
  \includegraphics[width=0.49\textwidth]{dr4_archive_001.pdf} & \includegraphics[width=0.49\textwidth]{dr4_archive_002.pdf}
 \\ Zeiss Triplet, Potsdam, 4921 plates & Carte du Ciel, Potsdam,  979 plates \\[6pt]
  \includegraphics[width=0.49\textwidth]{dr4_archive_003.pdf} & \includegraphics[width=0.49\textwidth]{dr4_archive_004.pdf}
 \\
 Great Schmidt Camera, Potsdam, 508 plates &  Great Schmidt Camera, Potsdam, 508 plates\\[6pt]
\includegraphics[width=0.49\textwidth]{dr4_archive_005.pdf} & 
  \includegraphics[width=0.49\textwidth]{dr4_archive_501.pdf} 
 \\
  Ross Camera, Potsdam, 64 plates &  Zeiss Double Astrograph, Vatican Observatory, 544 plates \\[6pt]
\end{tabular}
\vskip 0.5cm
\caption{\bf{Potsdam Archives}} 
\end{figure}         


\begin{figure}[h]
\begin{tabular}{cc}
  \includegraphics[width=0.5\textwidth]{dr4_archive_101.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_102.pdf}
 \\ Lippert-Astrograph, Hamburg, 8750 plates & Grosser Schmidt-Spiegel, Hamburg,  5323 plates \\[6pt]
  \includegraphics[width=0.5\textwidth]{dr4_archive_103.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_104.pdf}
 \\ 1m-Spiegelteleskop, Hamburg, 7643 plates & Hamburger Schmidt-Spiegel, Calar Alto,  3255 plates \\[6pt]
  \includegraphics[width=0.5\textwidth]{dr4_archive_105.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_106.pdf}
 \\ AG-Teleskop, Bonn, 754 plates & AG-Teleskop, Hamburg,  3529 plates \\[6pt]
  \includegraphics[width=0.5\textwidth]{dr4_archive_107.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_108.pdf}
 \\ Doppel-Reflektor, Hamburg, 1642 plates & ESO telescopes, La Silla,  2099 plates \\[6pt]
\end{tabular}
\vskip 0.5cm
\caption{\bf{Hamburg Archives I}} 
\end{figure}       


\pagebreak
\begin{figure}[h]
\begin{tabular}{cc}
  \includegraphics[width=0.5\textwidth]{dr4_archive_109.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_110.pdf}
 \\ Grosser Refraktor, Hamburg, 2602 plates & Kleiner Schmidt-Spiegel II, Hamburg, 1566 plates \\[6pt]
   \includegraphics[width=0.5\textwidth]{dr4_archive_111.pdf} & 
 \\ Schmidtsches Spiegelteleskop, Hamburg, 1746 plates & \\[6pt]
\end{tabular}
\vskip 0.5cm
\caption{\bf{Hamburg Archives II}} 
\end{figure}         


\begin{figure}[h]
\begin{tabular}{cc}
  \includegraphics[width=0.5\textwidth]{dr4_archive_202.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_203.pdf}
 \\Metcalf Telescope, South Africa, 2718 plates & Bamberg Southern Sky Patrol, South Africa, 12565 plates \\[6pt]
   \includegraphics[width=0.5\textwidth]{dr4_archive_204.pdf} & 
   \includegraphics[width=0.5\textwidth]{dr4_archive_205.pdf} 
 \\ Bamberg Southern Sky Patrol, New Zealand, 5266 plates & Bamberg Southern Sky Patrol, Argentina, 870 plates\\[6pt]
   \includegraphics[width=0.5\textwidth]{dr4_archive_206.pdf} & 
   \includegraphics[width=0.5\textwidth]{dr4_archive_207.pdf} 
 \\ Zeiss Objective, South Africa, 694 plates & Ross B Camera, South Africa, 698 plates\\[6pt]
    \includegraphics[width=0.5\textwidth]{dr4_archive_208.pdf} &   
 \\ Astrograph, Bamberg Northern Sky Patrol, 18865 plates & \\[6pt]
\end{tabular}
\vskip 0.5cm
\caption{\bf{Bamberg Archives}} 
\end{figure}  


\begin{figure}[h]
\begin{tabular}{cc}
  \includegraphics[width=0.5\textwidth]{dr4_archive_301.pdf} & \includegraphics[width=0.5\textwidth]{dr4_archive_401.pdf}
 \\Tartu Old Observatory, Tartu, 2275 plates &  Schmidt Telescope, Tautenburg, 4101 plates \\[6pt]
   \includegraphics[width=0.5\textwidth]{dr4_archive_501.pdf} & 
   % \includegraphics[width=0.5\textwidth]{dr4_archive_205.pdf} 
 \\ Zeiss Double Astrograph, Vatican Observatory, 544 plates & \\[6pt]
\end{tabular}
\vskip 0.5cm
\caption{\bf{Tartu, Tautenburg, Vatican Archives}} 
\end{figure}  

==> applause_plot_pdf.tex <==
\onecolumn
\section{Mollweide maps of observations per archive} 
\begin{figure}[h]
\begin{tabular}{cc}
  	\includegraphics[width=0.49\textwidth]{pdf/dr4_archive_001.pdf} & 
	\includegraphics[width=0.49\textwidth]{pdf/dr4_archive_002.pdf}
 \\[-11pt]
 	Zeiss Triplet, Potsdam, 4921 plates & Carte du Ciel, Potsdam,  979 plates 
  \\[1pt]
  	\includegraphics[width=0.49\textwidth]{pdf/dr4_archive_003.pdf} & 
	\includegraphics[width=0.49\textwidth]{pdf/dr4_archive_004.pdf}
 \\[-11pt]
 	Great Schmidt Camera, Potsdam, 508 plates &  Great Schmidt Camera, Potsdam, 508 plates
  \\[1pt]
	\includegraphics[width=0.49\textwidth]{pdf/dr4_archive_005.pdf} & 
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_101.pdf}  
 \\[-11pt]
  Ross Camera, Potsdam, 64 plates &   Lippert-Astrograph, Hamburg, 8750 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_102.pdf} & 
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_103.pdf} 
  \\[-11pt]
  Grosser Schmidt-Spiegel, Hamburg,  5323 plates & 1m-Spiegelteleskop, Hamburg, 7643 plates 
  \\[1pt]

\end{tabular}
% \vskip 0.5cm
% \caption{\bf{Applause Archives}} 
\end{figure}         
\pagebreak

\begin{figure}[h]
\begin{tabular}{cc}   
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_104.pdf} & 
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_105.pdf} 
  \\[-11pt] 
  Hamburger Schmidt-Spiegel, Calar Alto,  3255 plates & AG-Teleskop, Bonn, 754 plates 
  \\[1pt]
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_106.pdf} & 
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_107.pdf} 
  \\ [-11pt]
  AG-Teleskop, Hamburg,  3529 plates & Doppel-Reflektor, Hamburg, 1642 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_108.pdf} & 
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_109.pdf} 
  \\[-11pt]
   ESO telescopes, La Silla,  2099 plates & Grosser Refraktor, Hamburg, 2602 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_110.pdf} & 
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_111.pdf} 
  \\[-11pt]
   Kleiner Schmidt-Spiegel II, Hamburg, 1566 plates & Schmidtsches Spiegelteleskop, Hamburg, 1746 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_202.pdf} & 
   \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_203.pdf} 
  \\[-11pt] 
  Metcalf Telescope, South Africa, 2718 plates & Bamberg Southern Sky Patrol, South Africa, 12565 plates
  \\[1pt]

\end{tabular}
% \vskip 0.5cm
% \caption{\bf{Applause Archives}} 
\end{figure}         
\pagebreak

\begin{figure}[h]
\begin{tabular}{cc}    
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_204.pdf} & 
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_205.pdf} 
  \\[-11pt] 
  Bamberg Southern Sky Patrol, New Zealand, 5266 plates & Bamberg Southern Sky Patrol, Argentina, 870 plates
  \\[1pt]
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_206.pdf} & 
    \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_207.pdf} 
  \\ 
  Zeiss Objective, South Africa, 694 plates & Ross B Camera, South Africa, 698 plates
  \\[1pt]
     \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_208.pdf} &   
	 \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_301.pdf} 
  \\[1pt] 
  	Astrograph, Bamberg Northern Sky Patrol, 18865 plates & Tartu Old Observatory, Tartu, 2275 plates 
  \\[1pt]

  \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_401.pdf} &
  \includegraphics[width=0.5\textwidth]{pdf/dr4_archive_501.pdf}
 \\[1pt]
 	Schmidt Telescope, Tautenburg, 4101 plates & Zeiss Double Astrograph, Vatican Observatory, 544 plates 
 \\[1pt]

\end{tabular}
\vskip 0.5cm
\caption{\bf{Applause Archives}} 
\end{figure}         




==> applause_plot_png.tex <==
\onecolumn
\section{Mollweide maps of observations per archive} 
\begin{figure}[h]
\begin{tabular}{cc}
  	\includegraphics[width=0.49\textwidth]{png/dr4_archive_001.png} & 
	\includegraphics[width=0.49\textwidth]{png/dr4_archive_002.png}
 \\[-11pt]
 	Zeiss Triplet, Potsdam, 4921 plates & Carte du Ciel, Potsdam,  979 plates 
  \\[1pt]
  	\includegraphics[width=0.49\textwidth]{png/dr4_archive_003.png} & 
	\includegraphics[width=0.49\textwidth]{png/dr4_archive_004.png}
 \\[-11pt]
 	Great Schmidt Camera, Potsdam, 508 plates &  Great Schmidt Camera, Potsdam, 508 plates
  \\[1pt]
	\includegraphics[width=0.49\textwidth]{png/dr4_archive_005.png} & 
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_101.png}  
 \\[-11pt]
  Ross Camera, Potsdam, 64 plates &   Lippert-Astrograph, Hamburg, 8750 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_102.png} & 
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_103.png} 
  \\[-11pt]
  Grosser Schmidt-Spiegel, Hamburg,  5323 plates & 1m-Spiegelteleskop, Hamburg, 7643 plates 
  \\[1pt]

\end{tabular}
% \vskip 0.5cm
% \caption{\bf{Applause Archives}} 
\end{figure}         
\pagebreak

\begin{figure}[h]
\begin{tabular}{cc}   
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_104.png} & 
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_105.png} 
  \\[-11pt] 
  Hamburger Schmidt-Spiegel, Calar Alto,  3255 plates & AG-Teleskop, Bonn, 754 plates 
  \\[1pt]
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_106.png} & 
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_107.png} 
  \\ [-11pt]
  AG-Teleskop, Hamburg,  3529 plates & Doppel-Reflektor, Hamburg, 1642 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_108.png} & 
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_109.png} 
  \\[-11pt]
   ESO telescopes, La Silla,  2099 plates & Grosser Refraktor, Hamburg, 2602 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_110.png} & 
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_111.png} 
  \\[-11pt]
   Kleiner Schmidt-Spiegel II, Hamburg, 1566 plates & Schmidtsches Spiegelteleskop, Hamburg, 1746 plates 
  \\[1pt]
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_202.png} & 
   \includegraphics[width=0.5\textwidth]{png/dr4_archive_203.png} 
  \\[-11pt] 
  Metcalf Telescope, South Africa, 2718 plates & Bamberg Southern Sky Patrol, South Africa, 12565 plates
  \\[1pt]

\end{tabular}
% \vskip 0.5cm
% \caption{\bf{Applause Archives}} 
\end{figure}         
\pagebreak

\begin{figure}[h]
\begin{tabular}{cc}    
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_204.png} & 
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_205.png} 
  \\[-11pt] 
  Bamberg Southern Sky Patrol, New Zealand, 5266 plates & Bamberg Southern Sky Patrol, Argentina, 870 plates
  \\[1pt]
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_206.png} & 
    \includegraphics[width=0.5\textwidth]{png/dr4_archive_207.png} 
  \\ 
  Zeiss Objective, South Africa, 694 plates & Ross B Camera, South Africa, 698 plates
  \\[1pt]
     \includegraphics[width=0.5\textwidth]{png/dr4_archive_208.png} &   
	 \includegraphics[width=0.5\textwidth]{png/dr4_archive_301.png} 
  \\[1pt] 
  	Astrograph, Bamberg Northern Sky Patrol, 18865 plates & Tartu Old Observatory, Tartu, 2275 plates 
  \\[1pt]

  \includegraphics[width=0.5\textwidth]{png/dr4_archive_401.png} &
  \includegraphics[width=0.5\textwidth]{png/dr4_archive_501.png}
 \\[1pt]
 	Schmidt Telescope, Tautenburg, 4101 plates & Zeiss Double Astrograph, Vatican Observatory, 544 plates 
 \\[1pt]

\end{tabular}
\vskip 0.5cm
\caption{\bf{Applause Archives}} 
\end{figure}         



